Quantum Hoare Logic with Ghost Variables

Quantum Hoare logic allows us to reason about quantum programs. We present an extension of quantum Hoare logic that introduces "ghost variables" to extend the expressive power of pre-/postconditions. Ghost variables are variables that do not actually occur in the program and are allowed to have arbitrary quantum states (in a sense, they are existentially quantified), and be entangled with program variables. Ghost variables allow us to express properties such as the distribution of a program variable or the fact that a variable has classical content. And as a case study, we show how quantum Hoare logic with ghost variables can be used to prove the security of the quantum one-time pad.

==> macros.tex <==
\makeatletter

% \showafter{year}{month}{day}{text} evaluates to {text} starting from year/month/day
\newcommand\showafter[4]{%
  \ifnum\year>#1\relax
    #4% today.year > args.year
  \else
    \ifnum\year=#1\relax
    % today.year = args.year
      \ifnum\month>#2\relax
      % today.month > args.month
        #4%
      \else
        \ifnum\month=#2\relax
        % today.month = args.month
          \ifnum\day>#3\relax
          % today.day >= args.day
            #4%
          \else
            \ch@removeduplicatespace
          \fi
        \else
          \ch@removeduplicatespace
        \fi
      \fi
    \else
      \ch@removeduplicatespace
    \fi
  \fi}


\newcommand\TIlde{\Tilde}

\newcommand\pagelabel[1]{\phantomsection\label{#1}}

\DeclareRobustCommand\autorefshort[1]{%
  \def\lemmaautorefname{Lem.\!}%
  \autoref{#1},
  p.\,\pageref{#1}}

\newlistof{rule}{rule}{{List of rules}}
\renewcommand\cftruletitlefont{\section*}
\newcommand\rulestrut{}
\newcommand\rulespace{}
\newcommand\RULE[4][]{%
  \inferrule[\rulestrut{#2\ifx\norulelemmalink\undefined
    % \textsuperscript{\normalfont\tiny[\autorefshort{rule-lemma:#2}]}
    \fi}%
    \refstepcounter{rule}%
    \label{rule:#2}%
    \index{#2@\textsc{#2} (rule)}%
    \addcontentsline{rule}{rule}{\textsc{#2}%
      \ifx\@nil#1\@nil\else\space -- #1\fi}
  ]{#3}{#4}\rulespace%  
}
\newcommand\RULEX[4][]{%
  \inferrule[\rulestrut{#2}%
      \ifx\@nil#1\@nil\else\space -- #1\fi]{#3}{#4}\rulespace%  
}
\newenvironment{ruleblock}{%
  \begin{center}%
    \def\rulestrut{\vrule height 1.3\baselineskip width 0pt\relax}%
    \def\rulespace{\qquad}%
    \noindent
  }{%
  \end{center}}
  
\newcommand\refrule[1]{\hyperref[rule:#1]{\hbox{\textsc{#1}}} rule}
\newcommand\ruleref[1]{\hyperref[rule:#1]{rule \hbox{\textsc{#1}}}}
\newcommand\rulerefx[1]{\hyperref[rule:#1]{\hbox{\textsc{#1}}}}
\newcommand\Ruleref[1]{\hyperref[rule:#1]{Rule \hbox{\textsc{#1}}}}

\newenvironment{tinymatrix}{%
  \arraycolsep=1.4pt
  \tiny\begin{pmatrix}%
  }{%
  \end{pmatrix}} 

\mdfdefinestyle{proofstyle}{%
  backgroundcolor=black!4!white,
  innertopmargin=3pt,
  innerbottommargin=3pt,
  innerleftmargin=3pt,
  innerrightmargin=3pt,
  linewidth=0pt
}

\mdfdefinestyle{claimproofstyle}{%
  backgroundcolor=black!8!white,
  innertopmargin=0pt,
  innerbottommargin=3pt,
  innerleftmargin=3pt,
  innerrightmargin=3pt,
  leftmargin=10pt,
  rightmargin=10pt,
  % linewidth=0pt
}

  \newenvironment{proof}[1][]{%
    \begin{mdframed}[style=proofstyle]%
      \begin{trivlist}%
      \item \textit{Proof\ifx\proof#1\proof\else\ #1\fi. }%
      }{
        \qed\global\let\qed\qedmacro
      \end{trivlist}
    \end{mdframed}}%

  \newenvironment{claimproof}{%
    \let\qedbox\qedboxclaim
    \begin{mdframed}[style=claimproofstyle]%
      \begin{trivlist}%
      \item \textit{Proof of claim. }%
      }{
        \qed\global\let\qed\qedmacro
      \end{trivlist}
    \end{mdframed}}%

  \newenvironment{claimproofstart}{%
    \let\qedbox\qedboxclaim
    \begin{mdframed}[style=claimproofstyle]%
      \begin{trivlist}%
      \item \textit{Proof of claim. }%
      }{
      \end{trivlist}
    \end{mdframed}}%

  \newenvironment{claimproofend}{%
    \let\qedbox\qedboxclaim
    \begin{mdframed}[style=claimproofstyle]%
      \begin{trivlist}%
      \item%
      }{
        \qed\global\let\qed\qedmacro
      \end{trivlist}
    \end{mdframed}}%


% \shortonly{
% \newenvironment{claimproof}{%
%   \def\qed{\hfill\qedboxclaim}%
%   \begin{proof}[Proof of claim]}{\end{proof}}
% }

\newcommand\qedboxclaim{\ensuremath\diamond}
\newcommand\qedbox{\m@th$\Box$}
\newcommand\qedmacro{\hfill\qedbox}
\global\let\qed\qedmacro
\newcommand\skipqed{\global\let\qed\empty}
\newcommand\mathQED{\tag*{\qedbox}\skipqed}
\newcommand\txtrel[1]{\stackrel{\hskip-1in\text{\tiny#1}\hskip-1in}}
\newcommand\eqrefrel[1]{\txtrel{\eqref{#1}}}
\newcommand\starrel{\txtrel{$(*)$}}
\newcommand\starstarrel{\txtrel{$(**)$}}
\newcommand\tristarrel{\txtrel{$\scriptscriptstyle (\!*\!*\!*\!)$}}
\newcommand\fourstarrel{\txtrel{$\scriptscriptstyle (\!*\!*\!*\!*\!)$}}



\def\parenthesis@resizecommand@open{}
\def\parenthesis@resizecommand@close{}
\def\parenthesis@#1#2#3#4#5{%
  \global\let\parenthesis@resizecommand@open\empty
  \global\let\parenthesis@resizecommand@close\empty
  #1#3%
  {#5}%
  #2#4%
}
\DeclareRobustCommand\parenthesis[3]{%
  \expandafter\expandafter\expandafter
  \parenthesis@\expandafter\expandafter\expandafter{\expandafter\parenthesis@resizecommand@open\expandafter}\expandafter{\parenthesis@resizecommand@close}{#1}{#2}{#3}}


% #1=bigl #2=bigr #3=( #4=txt #5=) #6=txt #7=( #8=txt #9=)
\def\double@parenthesis@#1#2#3#4#5#6#7#8#9{%
  \global\let\parenthesis@resizecommand@open\empty
  \global\let\parenthesis@resizecommand@close\empty
  #1#3{#4}#2#5%
  {#6}%
  #1#7{#8}#2#9%
}

\DeclareRobustCommand\doubleParenthesis[7]{%
  \expandafter\expandafter\expandafter
  \double@parenthesis@\expandafter\expandafter\expandafter{\expandafter\parenthesis@resizecommand@open\expandafter}\expandafter{\parenthesis@resizecommand@close}{#1}{#2}{#3}{#4}{#5}{#6}{#7}}


\DeclareRobustCommand\resize@next@paren[2]{%
  \gdef\parenthesis@resizecommand@open{#1}%
  \gdef\parenthesis@resizecommand@close{#2}%
}

\newcommand\paren{\parenthesis()}
\newcommand\braces{\parenthesis\{\}}
\newcommand\bracket{\parenthesis[]}

\newcommand\pb{\resize@next@paren\bigl\bigr}
\newcommand\pbb{\resize@next@paren\biggl\biggr}
\newcommand\plr{\resize@next@paren\left\right}
\newcommand\pB{\resize@next@paren\Bigl\Bigr}
\newcommand\pBb{\resize@next@paren\biggl\biggr}


\newcommand\bit{\{0,1\}}
\newcommand\bits[1]{\bit^{#1}}
\newcommand\fsq{\tfrac1{\sqrt2}}
  
\declare{macro=\setN, code=\mathbb N,
  description={Natural numbers $1,2,3,\dots$}}
\declare{macro=\setR, code=\mathbb R,
  description={Real numbers}}
\declare{macro=\setC, code=\mathbb C,
  description={Complex numbers}}

\declare{macro=\xx, code=\mathbf x, wrap=group,
  placeholder={\xx,\yy,\zz},
  description={Program variable}}
\newcommand\yy{{\mathbf y}}
\newcommand\zz{{\mathbf z}}

\declare{macro=\vv, code=\mathbf v, wrap=group,
  placeholder={\vv,\ww},
  description={Variable}}
\newcommand\ww{{\mathbf w}}

\declare{macro=\ee, code=\mathbf e,
  placeholder={\ee},
  description={Entangled ghost variable}}

\declare{macro=\uu, code=\mathbf u,
  placeholder={\uu},
  description={Unentangled ghost variable}}

\declare{macro=\gggg, code=\mathbf g,
  placeholder={\gggg},
  description={Ghost variable}}


\declare{macro=\XX, code=\mathbf X,
  placeholder={\XX,\YY,\ZZ},
  description={List/set of program variables}}
\newcommand\YY{\mathbf Y}
\newcommand\ZZ{\mathbf Z}
\declare{macro=\UU, code=\mathbf U,
  description={List/set of unentangled ghost variables}}
\declare{macro=\EE, code=\mathbf E,
  description={List/set of entangled ghost variables}}
\declare{macro=\GG, code=\mathbf G,
  description={List/set of ghost variables}}
\declare{macro=\VV, code=\mathbf V,
  placeholder={\VV,\WW},
  description={List/set of variables}}
\newcommand\WW{\mathbf W}

\declare{macro=\ket, argspec=[1], code=\parenthesis\lvert\rangle{#1},
  placeholder=\ket x,
  description={Basis state $x$}}
\declare{macro=\bra, argspec=[1], code=\parenthesis\langle\rvert{#1},
  placeholder=\bra x,
  description={Adjoint of $\ket x$, i.e., $\adj{\ket x}$}}

\declare{macro=\elltwo, argspec=[1], code={\ell^2(#1)},
  placeholder=\elltwo X,
  description={Hilbert space with basis indexed by $X$}}
\declare{macro=\elltwov, argspec=[1], code={\ell^2\parenthesis[]{#1}},
  placeholder=\elltwov\VV,
  description={Pure quantum assignments on $\VV$}}

\declare{macro=\mm, code=\mathsf m, wrap=group,
  description={An assignment}}

\declare{macro=\tensor, code=\otimes,
  placeholder={A\otimes B},
  description={Tensor product of vectors/operators/spaces $A$ and $B$}}

\declare{macro=\opon, argspec=[2], code={#1\,\mathbf{on}\,#2},
  placeholder=\opon U\VV,
  description={Operator $U$ applied to variables $\VV$}}
\newcommand\oponp[2]{\paren{\opon{#1}{#2}}}

\declare{macro=\PA, code=\mathsf A,
  placeholder={\PA,\PB,\PC},
  description={(Quantum) predicates}}

\newcommand\PB{\mathsf B}
\newcommand\PC{\mathsf C}

\declare{macro=\norm, argspec=[1], code={\parenthesis\lVert\rVert{#1}},
  placeholder=\norm \psi, description={Norm of vector $\psi$}}

\declare{macro=\abs, argspec=[1], code={\parenthesis\lvert\rvert{#1}},
  placeholder=\abs x, description={Absolute value/cardinality}}

\declare{macro=\quantin, code=\in_{\mathfrak q},
  placeholder=\VV\quantin S,
  description={Predicate: $\VV$ has a value in $S$}}

\declare{macro=\SPAN, code={\operatorname{span}},
  placeholder=\SPAN A,
  description={Span, smallest subspace containing $A$}}

\declare{macro=\quanteq, code={=_\mathfrak q},
  placeholder={\VV\quanteq\psi},
  description={Predicate: $\VV$ is in state $\psi$}}

\declare{macro=\QUANTEQ, code={\equiv_\mathfrak q},
  placeholder={\WW\QUANTEQ\WW'},
  description={Predicate: $\WW$ and $\WW'$ are in the same state}}

\declare{macro=\CLASSEQ, code={\equiv_\mathfrak{c\mkern-1mu l}},
  placeholder={\VV\CLASSEQ\VV'},
  description={Predicate: $\VV$ and $\VV'$ are classically in the same state}}

\declare{macro=\SWAP, code=\mathsf{SWAP},
  description={Unitary that swaps $\WW$ and $\WW'$}}

\declare{macro=\top,
  description={Predicate: always satisfied}}
\declare{macro=\zero, code=\bot,
  description={Predicate: never satisfied}}

\declare{macro=\wedge,
  placeholder={\PA\wedge\PB,\ \PA,\PB},
  description={Intersection of predicates (conjunction)}}

\declare{macro=\vee,
  placeholder={\PA\vee\PB},
  description={Sum of predicates (disjunction)}}

\declare{macro=\fv, code=\mathsf{fv},
  placeholder=\fv(a),
  description={Free variables of predicate/program $a$}}

\declare{macro=\bc, code=\pmb{\mathfrak c}, nopage=true,
  placeholder={\bc,\bd},
  description={A program}}
\newcommand\bd{\pmb{\mathfrak d}}

\declare{macro=\apply, argspec=[2], code={{\applykw}\ #1\ \underline{\mathbf{to}}\ #2},
  placeholder=\apply U\VV,
  description={Program: Apply $U$ to variables $\VV$}}
\newcommand\applykw{\underline{\mathbf{apply}}}

\declare{macro=\init, argspec=[1], code={\underline{\mathbf{init}}\ #1},
  placeholder=\init\xx,
  description={Program: Initialize $\xx$ with $\ket0$}}

\declare{macro=0,
  description={Default value (in every variable type)}}

\declare{macro=\ifte, argspec=[3], code={\underline{\mathbf{if}}\ #1\ \underline{\mathbf{then}}\ #2\ \underline{\mathbf{else}}\ #3},
  placeholder=\ifte \xx\bc\bd,
  description={Program: If (conditional)}}

\declare{macro=\while, argspec=[2], code={\underline{\mathbf{while}}\ #1\ \underline{\mathbf{do}}\ #2},
  placeholder=\while\xx\bc,
  description={Program: While (loop)}}

\declare{macro=;,
  placeholder=\bc;\bd,
  description={Program: execute $\bc$ then $\bd$}}

\declare{macro=\SKIP, code=\underline{\mathbf{skip}},
  description={Program: does nothing}}
  
\declare{macro=\denot, argspec=[1], code={\parenthesis\llbracket\rrbracket{#1}},
  placeholder={\denot \bc},
  description={Denotation of a program $\bc$}}

\declare{macro=\proj, argspec=[1], code={\mathsf{proj}\parenthesis(){#1}},
  placeholder=\proj \psi,
  description={Projector onto $\psi$, i.e., $\psi\adj \psi$}}

\declare{macro=\adj, argspec=[1], code=#1^*,
  placeholder={\adj a},
  description={Adjoint of operator/vector $a$}}
\newcommand\adjp[1]{\adj{\paren{#1}}}

\declare{macro=\tr, code=\operatorname{tr},
  placeholder=\tr M,
  description={Trace of matrix/operator $M$}}

%\declare{macro=\density, argspec=[1], code=\mathbf S(#1),
%  placeholder={\density X},
%  description=Mixed states / density operators on $\elltwo X$}

% \declare{macro=\densityv, argspec=[1], code=\mathbf S[#1],
%   placeholder={\densityv\VV},
%   description=Mixed quantum memories (mixed states / density operators on $\elltwov\VV$)}

\declare{macro=\id, code=\mathsf{id},
  description=Identity}

\declare{macro=\restrict, argspec=[1], code=\mathord{\downarrow_{#1}},
  placeholder=\restrict i(\rho),
  description=Mixed state restricted to measurement outcome $i$}

\declare{macro=\inits, argspec=[2],
  code={#1\stackrel{{\scriptstyle{\smash{\mathfrak q}}}}\leftarrow #2},
  placeholder=\inits\XX\psi,
  description={Program: Initialize $\XX$ with quantum state $\psi$}}

\declare{macro=\initc, argspec=[2],
  code={#1\leftarrow #2},
  placeholder=\initc\XX z,
  description={Program: Initialize $\XX$ with classical value $z$}}

\declare{macro=\measure, argspec=[2], code=#1\leftarrow \underline{\mathbf{measure}}\ #2,
  placeholder=\measure\yy\XX,
  description={Program: Measure $\XX$ in computational basis, assign outcome to $\yy$}}

\declare{macro=\measuref, argspec=[1], code=\underline{\mathbf{measure}}\ #1,
  placeholder=\measuref\XX,
  description={Program: Measure $\XX$ in computational basis, forget outcome}}

\declare{macro=\sample, argspec=[2], code={#1\stackrel{{\scriptstyle{}\smash\$}}\leftarrow #2},
  placeholder=\sample \XX D,
  description={Program: Sample $\XX$ according to distribution $D$}}

\declare{macro=\CNOT, code=\mathsf{CNOT},
  description={(Generalized) CNOT}}

\declare{macro=\hl, argspec=[3],
  code={\doubleParenthesis\{{#1}\}{\,#2\,}\{{#3}\}},
  placeholder=\hl \PA\bc\PB,
  description={Hoare judgment}}
\newcommand\hlfrag[1]{\braces{#1}}

\declare{macro=\suppo, code=\operatorname{\mathbf{supp}},
  placeholder=\suppo M,
  description={Support of an operator $M$}}

\declare{macro=\suppd, code=\operatorname{\mathrm{supp}},
  placeholder=\suppd D,
  description={Support of a distribution $D$}}

\declare{macro=\sats, argspec=[2], code={#1\vDash#2},
  placeholder=\sats\rho\PA,
  description={Mixed quantum memory $\rho$ satisfies predicate $\PA$}}


\declare{macro=\im, code=\operatorname{im},
  placeholder=\im M,
  description={Image of operator $M$}}

\declare{macro=\partr, argspec=[1], code=\tr_{#1},
  placeholder=\partr{\VV} \rho,
  description={Partial trace (removing variables $\VV$)}}

\declare{macro=\psiD, argspec=[1], code=\psi_{#1},
  placeholder=\psiD D,
  description={State encoding the distribution $D$}}

\declare{macro=\psiDD, argspec=[1], code=\psi_{#1#1},
  placeholder=\psiDD D,
  description={State encoding the distribution $D$ (on two variables)}}

\declare{macro=\distr, argspec=[2], code=\mathbf{distrib}\paren{#1,#2},
  placeholder=\distr\XX D,
  description={Predicate: $\XX$ has distribution $D$}}

\declare{macro=\uniform, argspec=[1], code=\mathbf{uniform}\paren{#1},
  placeholder=\uniform\XX,
  description={Predicate: $\XX$ has uniform distribution}}

\declare{macro=\class, argspec=[1], code=\mathbf{class}\paren{#1},
  placeholder=\class\XX,
  description={Predicate: $\XX$ is classical}}

\declare{macro=\separable, argspec=[1], code=\mathbf{separable}\paren{#1},
  placeholder=\separable\XX,
  description={Predicate: $\XX$ is separable from all other variables}}

\declare{macro=\psubst, argspec=[3], code=#1\braces{#2/#3},
  placeholder=\psubst\PA\vv\ww,
  description={Predicate $\PA$ with $\ww$ substituted by $\vv$}}
\newcommand\psubstii[5]{#1\braces{#2/#3,#4/#5}}

\declare{macro=\impl, code=\Rrightarrow,
  placeholder=\PA\impl\PB,
  description={``Implication'' of predicates}}

\declare{macro=\oppred, argspec=[2], code=#1\cdot#2,
  placeholder=\oppred M\PA,
  description={Operator $M$ applied to subspace $\PA$}}
\newcommand\oppredp[2]{\paren{\oppred{#1}{#2}}}

\declare{macro=\dotcup, code=\mathbin{\mathaccent\cdot\cup}, nopage=true,
  description={Disjoint union}}

\declare{macro=\Urename, argspec=[2], code=U_{#1\to#2}, 
  placeholder=\Urename\VV\WW,
  description={Rename variables $\VV$ into $\WW$}}

\declare{macro=\Ucopy, argspec=[2], code=U_{\mathsf{copy},#1\to#2}, 
  placeholder=\Ucopy\VV\WW,
  description={Copies classically from $\VV$ into $\WW$}}

% \declare{macro=\Erename, argspec=[2], code=\mathcal E_{#1\to#2}, 
%   placeholder=\Erename\VV\WW,
%   description={Rename variables $\VV$ into $\WW$}}

\declare{macro=\rank, code=\operatorname{rank},
  placeholder=\rank M,
  description={Rank of operator $M$}}

\declare{macro=\XXall, code=\XX^{\mathbf{all}},
  description={Set of program variables that can be used in the execution of a program}}

\declare{macro=\UX, argspec=[2], code={#1}^{\bracket{#2}},
  placeholder=\UX U\XX,
  description={Unitary $U_i$ controlled by $\XX$}}

\declare{macro=\PX, argspec=[2], code={#1}^{\bracket{#2}},
  placeholder=\PX \PA\XX,
  description={Predicate $\PA_i$ depending on $\XX$}}

\declare{macro=\pauliZ, code=Z,
  description={Pauli-Z operator}}

\declare{macro=\pauliX, code=X,
  description={Pauli-X operator}}

\declare{macro=\Keygen, code=\mathsf{Keygen},
  description={Key generation algorithm of the QOTP}}

\declare{macro=\Enc, code=\mathsf{Enc},
  description={Encryption algorithm of the QOTP}}

\declare{macro=\Enchalf, code=\mathsf{Enc_{1/2}},
  description={Encryption algorithm of $\frac12$QOTP}}

\declare{macro=\Dec, code=\mathsf{Dec},
  description={Decryption algorithm of the QOTP}}

\declare{macro=\rhl, argspec=[4],
  code={\doubleParenthesis\{{#1}\}{\,#2\,\sim\,#3\,}\{{#4}\}},
  placeholder=\rhl \PA\bc\bd\PB,
  description={Relational Hoare judgment}}

\declare{macro=\progvars, argspec=[1], code={\mathsf{progvars}(#1)},
  placeholder=\progvars\VV,
  description={Set of program variables in $\VV$}}

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "ghost"
%%% End:

